Doubly unfolded adjacency spectral embedding of dynamic multiplex graphs

Many real-world networks evolve dynamically over time and present different types of connections between nodes, often called layers. In this work, we propose a latent position model for these objects, called the dynamic multiplex random dot product graph (DMPRDPG), which uses an inner product between layer-specific and time-specific latent representations of the nodes to obtain edge probabilities. We further introduce a computationally efficient spectral embedding method for estimation of DMPRDPG parameters, called doubly unfolded adjacency spectral embedding (DUASE). The DUASE estimates are proved to be both consistent and asymptotically normally distributed. A key strength of our method is the encoding of time-specific node representations and layer-specific effects in separate latent spaces, which allows the model to capture complex behaviors while maintaining relatively low dimensionality. The embedding method we propose can also be efficiently used for subsequent inference tasks. In particular, we highlight the use of the ISOMAP algorithm in conjunction with DUASE as a way to efficiently capture trends and global changepoints within a network, and the use of DUASE for graph clustering. Applications on real-world networks describing geopolitical interactions between countries and financial news reporting demonstrate practical uses of our method.

==> Sections/background.tex <==

\section{Background} 
Our work builds on a number of concepts in the existing literature in particular it may be helpful for some readers to briefly discuss the some core concepts in graph analysis and foundational models related to our work. One of the foundational models that is used to describe network activity is the concept of the latent position model (LPM) or Latent Space Model (LSM). In this model each node $i \in \{1, \dots, n \}$ is equipped with a set of latent features represented by a vector $x_i$ in some low-dimensional space (typically $\mathbb{R}^d$ where $d << n$). These vectors fully characterize the behavior of the network through a kernel function $\kappa(\cdot)$. Concretely the probability of a link between node $i$ and node $j$ is given as 

$$\mathbb{P}[A_{i,j} = 1 ] = \kappa\left( x_i, x_j \right)$$

This model greatly simplifies the complexity of the setting as the general case of $n^2$ pairwise connection probabilities is fully characterized by $n \times d$ latent position coordinates. This compression makes graph inference a theoretically tractable problem in settings where the link function is known (or the case where a sufficiently accurate link function can be found). In the setting where $\kappa(x_i, x_j) \defeq x_i \cdot x_j$ we refer to the model as a random dot product graph (RDPG). The RDPG will the be the core of the model we present here as it is among the most widely studied and well-developed models which includes a rich literature including both consistency \cite{sussman2013consistent}  and distributional results \cite{tang2018limit} \cite{athreya2016limit}. In particular, our work builds on a multi-layer extension of the RDPG \cite{jones2021multilayer} where a shared set of nodes is able to exhibit connectivity through multiple ``connection types" which allows the model to describe a richer class of behaviors. \newline



Before discussing our model and results it will also be helpful for many readers to briefly discuss the concept of a graph embedding and highlight some of the work that has been done in the field. The concept of a graph embedding in the general sense refers of to a low dimensional representation that retains much of the structure of the inherently complex original graph. In the case of a RDPG or extensions thereof this generally translates to the problem of estimating the node latent positions based on observed network connectivity. To this end a number of streams of research have emerged most notably including spectral methods and ML-based methods \cite{perozzi2014deepwalk} \cite{grover2016node2vec}. Within the setting of spectral methods we can draw a distinction between standard spectral methods and tensor-based methods. Tensor based methods typically organize graph structures such as the adjacency matrix or Laplacian into a Tensor and employ or a higher order generalization of singular value decomposition to this object. They are often used to analyze generalizations of graphs in which connections occur between varying numbers of numbers but there may be merit in using similar methods to analyze dynamic or multiplex graphs where adjacency matrices have been aggregated into a higher dimensional structure. In the context of standard spectral embedding methods one of the foundational techniques used is adjacency spectral embedding (ASE) \cite{sussman2012consistent} where the scaled eigenvectors of the graph adjacency matrix $\Amat$ are used to obtain a latent position estimate. In the setting of multi-layer graphs there are several prominent methodologies in the spectral embedding regime including omnibus spectral emdedding (OSE) \cite{levin2017central}, mean adjacency spectral embedding (MASE) and unfolded adjacency spectral embedding (UASE) \cite{gallagher2021spectral}. For an in-depth overview of inference methods for RDPGs readers are directed to \cite{athreya2018statistical}.



==> Sections/existing_results.tex <==
\section{Existing Results}

\subsection{Multivariate Lendeberg-Feller CLT}
\begin{theorem}\label{LindebergFeller}
Suppose $y_{n,i} \in \mathbb{R}^k$ are independent but not necessarily identically distributed with finite means $\mu_{n,i} = \mathbb{E}[y_{n,i}]$ and variance matrices $\mat{V}_{n,i} = \mathbb{E}[(y_{n,i} - \mu_{n,i})(y_{n,i} - \mu_{n,i})^\intercal]$. Set $\overline{\mat{V_n}} = \frac{1}{n} \sum_{i=1}^n \mat{V}_{n,i}$ and $\nu_n^2 = \lambda_{min}(\overline{\mat{V}_n})$. If $\nu_n^2 > 0$ and for all $\epsilon > 0$ the Lindeberg condition is satisfied:

$$\lim_{n \to \infty} \frac{1}{n \nu_n^2} \sum_{i=1}^n \mathbb{E} \left( \norm{y_{n,i} - \mu_{n,i}}^2 1\left( \norm{y_{n,i} - \mu_{n,i}}^2 \geq \epsilon n \nu_n^2 \right)\right) = 0$$

then as $n \to \infty$
$$\bar{\mat{V_n}}^{-1/2} n^{1/2} (\bar{y} - \mathbb{E}\left(\bar{y} \right) \to \mathcal{N} \left(0, \mat{I}_k \right)$$.
\end{theorem}

\subsection{Matrix Bernstein Theorem 1.6.2 \cite{tropp2015introduction}}
\begin{theorem}\label{MatrixBernstein}
Let $\mat{S_1}, \dotsm \mat{S_n}$ be independent, centered random matrices with common dimension $d_1 \times d_2$ and assume that each one is uniformly bounded 
$$\mat{E} \left[\mat{S_k} \right]= \mat{0} \hspace{1cm} \norm{\mat{S_k}} \leq  L$$
for each $k = 1,\dots, n$. Introduce the sum 
$$\mat{Z} = \sum_{k=1}^{n} \mat{S_k}$$ and let $v(\mat{Z})$ denote the matrix variance statistic of the sum: 
$$v(\mat{Z}) = \max \left( \norm{\mat{E}\left[ \mat{Z} \mat{Z}^\intercal\right]}, \norm{\mat{E}\left[ \mat{Z}^\intercal \mat{Z}\right]} \right).$$
Then 
$$\mathbb{P} \left[ \norm{\mat{Z}} \geq t\right] \leq (d_1 + d_2) \exp \left(\frac{-t^2/2}{v(\mat{Z}) + Lt/3} \right).$$
\end{theorem}

==> Sections/technical_note.tex <==

%\subsection{ISOMAP and the Euclidean Mirror}

%\subsection{Analysis of Empirical Data}


%\subsection{A Note on the Scaling of $\hat{\Xmat}$ and $\hat{\Ymat}$}

It is important to note that the true scale of $\Xmat$ and $\Ymat$ are fundamentally unidentifiable as any scaling of $\Xmat$ by a constant factor $c$ and a corresponding scaling of $\Ymat$ by $c^{-1}$ produces an identical matrix $\Pmat$. % and therefore identical network activity. 
The scale of the estimates obtained via DUASE will be a function of both $\Kn$ and $\Tn$. In particular, the scaling of each $\hXm^k$ will be or order $\Tn^{1/4}\Kn^{-1/4}$ while the scaling of each $\hYm^t$ is of order $\Kn^{1/4}\Tn^{-1/4}$. As such, a corresponding rescaling can be done in practice to obtain estimates for the left and right embedding that are of approximately equal magnitude. 

%\section{Extensions and Future Work}

%\subsection{Stability Guarantees for DUASE}

%\subsection{Gaussian Process Modelling in the Embedding Space}

% One of the key strengths of DUASE is that it obtains a joint representation for all layers of a multiplex graph and its corresponding evolution through time. This creates the concept of a single time-varying trajectory that succinctly describes the evolution of network behavior. Such a structure may lend itself to existing low-dimensional modelling techniques such as classical time series methods Gaussian process models.  

%\subsection{Extension of Euclidean Mirror Theory to the Multiplex Setting}
